Distributed Dynamic Economic Dispatch using Alternating Direction Method of Multipliers

With the proliferation of distributed energy resources and the volume of data stored due to advancement in metering infrastructure, energy management in power system operation needs distributed computing. In this paper, we propose a fully distributed Alternating Direction Method of Multipliers (ADMM) algorithm to solve the distributed economic dispatch (ED) problem, where the optimization problem is fully decomposed between participating agents. In our proposed framework, each agent estimates the dual variable and the average of the total power mismatch of the network using dynamic average consensus, which replaces the dual updater in the traditional ADMM with a distributed alternative. Unlike other distributed ADMM, the proposed method does not rely on any specific assumption and captures the real-time demand change. The algorithm is validated successfully via case studies for IEEE 30-bus and 300-bus test systems with the penetration of solar photovoltaic.

==> ADMM MIT/figures_code.tex <==
%% Figures 1 ========================================================================
% sum(Pg) - sum(Pd)
\begin{figure}[h!]
    \begin{minipage}{1\linewidth}
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/30bus_figure_2.eps}
        \end{minipage}
        \vfill
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/300bus_figure_2.pdf}
        \end{minipage}
    \end{minipage}
    \caption{(a) and (d):Network's generation following demand  for IEEE 30-bus and 300-bus respectively;(b) and (e) are magnified version at the beginning , and (c) and (f) in the middle when the demand changed for 30-bus case and 300-bus respectively}
    \label{fig:300bus_Pgen_Pdem}
\end{figure}
%% Figures 2 ========================================================================
% Lambda Consensus
\begin{figure}[h!]
    \begin{minipage}{1\linewidth}
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/30bus_figure_1.pdf}
        \end{minipage}
        \vfill
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/300bus_figure_1.pdf}
        \end{minipage}
    \end{minipage}
    %\caption{Top: Market price consensus on IEEE 300-bus; bottom left: plot in a logarithmic scale in order to capture the convergence's dynamic of the algorithm ; bottom right: the convergence dynamics magnified when the demand changed}
    \caption{(a) and (d):Consensus on market price for IEEE 30-bus and 300-bus respectively;(b) is magnified version at the beginning for 30-bus and (e) is the plot in a logarithmic scale in order to capture the convergence's dynamic of the algorithm for 300-bus; (c) and (f) in the middle as demand changed for 30-bus and 300-bus respectively}
    \label{fig:300bus_lambda}
\end{figure}


%% Figures 3 ========================================================================
% Pg*
\begin{figure}[h!]
    \begin{minipage}{1\linewidth}
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/30bus_figure_3.eps}
            \caption{Generators output for  IEEE 30-bus}
            \label{fig:30bus_Pout}
        \end{minipage}
        \vfill
        %\begin{minipage}{1\linewidth}
          %  \includegraphics[width=\linewidth]{figures/118bus_figure_3.eps}
          %  \caption{Generators output IEEE 118 bus}
          %  \label{fig:118bus_figure_3}
       % \end{minipage}%
       % \vfill
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/300bus_figure_3.pdf}
            \caption{Generators output for IEEE 300-bus}
            \label{fig:300bus_Pout}
        \end{minipage}
    \end{minipage}
\end{figure}

%% Figures 4 ========================================================================
% average(Pgd)
\begin{figure}[h!]
    \begin{minipage}{1\linewidth}
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/30bus_figure_4.pdf}
            \caption{Average power mismatch in IEEE 30-bus}
            \label{fig:30bus_Pgd}
        \end{minipage}
       % \vfill
       % \begin{minipage}{1\linewidth}
          %  \includegraphics[width=\linewidth]{figures/118bus_figure_4.eps}
          %  \caption{Average power mismatch IEEE 118 bus}
          %  \label{fig:118bus_figure_4}
       % \end{minipage}%
        \vfill
        \begin{minipage}{1\linewidth}
            \includegraphics[width=\linewidth]{figures/300bus_figure_4.pdf}
            \caption{Average power mismatch IEEE 300-bus}
            \label{fig:300bus_Pgd}
        \end{minipage}
    \end{minipage}
\end{figure}

%% Figures 5 ========================================================================
% PV irradiance
\begin{comment}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/30bus_figure_5.eps}
    \caption{Solar power profile}
    \label{fig:30bus_figure_5}
\end{figure}
\end{comment}
%% ==================================================================================

==> ADMM MIT/table_results.tex <==
%% Results----------------------------------------------------------

\begin{table*}[H]

\centering
\caption{$\lambda$ convergence table } 
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{Test} & {Total} & {Total} & \multicolumn{2}{c|}{Initial Convergence} & \multicolumn{2}{c|}{Subsequent Convergence}\\
\cline{4-7} {Case} & {Time} & {Iteration} & \multicolumn{1}{l|}{\# iteration} & \multicolumn{1}{l|}{Time [sec]} & \multicolumn{1}{l|}{\# iteration} & \multicolumn{1}{l|}{Time [sec]} \\ \hline
Case 30  &  22.4 & 1e6 & 1250 & 0.03 & 1000 & 0.022\\ \hline
Case 118 & 51.61 & 1e6 & 20000 & 1.03 & 17500 & 0.903 \\ \hline
Case 300 & 136.614 & 1e6 & 70000 & 9.56 & 5500 & 0.751                           \\ \hline
\end{tabular}
\label{table: lambda convergence}

\end{table*}
%--------------------------------------------------------------

==> table_results.tex <==
%% Results----------------------------------------------------------

\begin{table*}[H]

\centering
\caption{$\lambda$ convergence table } 
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{Test} & {Total} & {Total} & \multicolumn{2}{c|}{Initial Convergence} & \multicolumn{2}{c|}{Subsequent Convergence}\\
\cline{4-7} {Case} & {Time} & {Iteration} & \multicolumn{1}{l|}{\# iteration} & \multicolumn{1}{l|}{Time [sec]} & \multicolumn{1}{l|}{\# iteration} & \multicolumn{1}{l|}{Time [sec]} \\ \hline
Case 30  &  22.4 & 1e6 & 1250 & 0.03 & 1000 & 0.022\\ \hline
Case 118 & 51.61 & 1e6 & 20000 & 1.03 & 17500 & 0.903 \\ \hline
Case 300 & 136.614 & 1e6 & 70000 & 9.56 & 5500 & 0.751                           \\ \hline
\end{tabular}
\label{table: lambda convergence}

\end{table*}
%--------------------------------------------------------------
